Bridging Functional Correctness and Runtime Efficiency Gaps in LLM-Based Code Translation

While large language models (LLMs) have greatly advanced the functional correctness of automated code translation systems, the runtime efficiency of translated programs has received comparatively little attention. With the waning of Moore's law, runtime efficiency has become increasingly important for program quality, alongside functional correctness. Our preliminary study reveals that LLM-translated programs often run slower than human-written ones, and this issue cannot be remedied through prompt engineering alone. Therefore, our work proposes SwiftTrans, a code translation framework comprising two key stages: (1) Multi-Perspective Exploration, where MpTranslator leverages parallel in-context learning (ICL) to generate diverse translation candidates; and (2) Difference-Aware Selection, where DiffSelector identifies the optimal candidate by explicitly comparing differences between translations. We further introduce Hierarchical Guidance for MpTranslator and Ordinal Guidance for DiffSelector, enabling LLMs to better adapt to these two core components. To support the evaluation of runtime efficiency in translated programs, we extend existing benchmarks, CodeNet and F2SBench, and introduce a new benchmark, SwiftBench. Experimental results across all three benchmarks show that SwiftTrans achieves consistent improvements in both correctness and runtime efficiency.

==> sec/ReproducibilityStatement.tex <==
\section*{Reproducibility Statement}
We have taken extensive measures to ensure the reproducibility of our results.
All benchmarks used in this work (CodeNet, F2SBench, and \ourbench) are publicly available or will be released upon acceptance of this paper.
We provide full details of experimental settings, including training data construction, prompt templates, and evaluation metrics.
Implementation details such as the number of demonstrations per perspective, the depth of hierarchical acceleration, and the loss functions used for optimization are described in Sec.~\ref{sec:Implementation Details}.
For runtime evaluation, we employed the Judge0 execution sandbox, a widely used open-source platform, as shown in Sec.~\ref{sec:Metric Design}.
To further support reproducibility, we will release the source code for our \ourapproach framework, including data processing scripts, training configurations, and evaluation pipelines.
These materials will allow other researchers to replicate our experiments and validate our findings across different hardware setups.
